Experimental study of pedestrian flow through a T-junction

In this study, series of experiments under laboratory conditions were carried out to investigate pedestrian flow through a T-junction, i.e., two branches merging into the main stream. The whole duration of the experiments was recorded by video cameras and the trajectories of each pedestrian were extracted using the software Petrack from these videos. The Voronoi method is used to resolve the fine structure of the fundamental diagram and spatial dependence of the measured quantities from trajectories. In our study, only the data in the stationary state are used by analyzing the time series of density and velocity. The density, velocity and specific flow profiles are obtained by refining the size of the measurement area (here 10 cm \times 10 cm are adopted). With such a high resolution, the spatial distribution of density, velocity and specific flow can be obtained separately and the regions with higher value can be observed intuitively. Finally, the fundamental diagrams of T-junction flow is compared in three different locations. It is shown that the fundamental diagrams of the two branches match well. However, the velocities in front of the merging are significantly lower than that in the main stream at the same densities. After the merging, the specific flow increases with the density \rho till 2.5 m-2. While in the branches, the specific flow is almost independent of the density between \rho = 1.5 m-2 and 3.5 m-2

==> ctextemp_referenc.tex <==
\def\CTeXPreproc{Created by ctex v0.2.12, don't edit!}%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% "computer science"
%
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%

%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
% Non-BibTeX users please use
\begin{thebibliography}{99.}
%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references
%
\bibitem{Appert-Rolland2009}
C.~Appert-Rolland, F.~Chevoir, P.~Gondret, S.~Lassarre, J.-P.
Lebacque, and M.~Schreckenberg (2009)
\newblock {\em {Traffic and Granular Flow '07}} (Berlin: Springer)

\bibitem{Bandini2010}
S.~Bandini, S.~Manzoni, H.~Umeo, and G.~Vizzari (2010)
\newblock {\em {Workshop on Crowds and CA, ACRI 2010: Cellular Automata 9th International Conference on Cellular
  Automata for Reseach and Industry}} (Berlin: Springer), Italy

\bibitem{Klingsch2010}
W.~W.~F. Klingsch, C.~Rogsch, A.~Schadschneider, and
M.~Schreckenberg (2010)
\newblock {\em {Pedestrian and Evacuation Dynamics 2008}}. Springer-Verlag
  Berlin Heidelberg

\bibitem{Schadschneider2009}
A.~Schadschneider, H.~Kl\"upfel, T.~Kretz, and A.~Rogsch,
C.and~Seyfried (2009)
\newblock {Fundamentals of Pedestrian and Evacuation Dynamics}.
In: {\em {Multi-Agent Systems for Traffic and Transportation
Engineering}}, pp. 124--154. IGI Global, Hershey, Pennsylvania, USA

\bibitem{Schadschneider2009c}
A.~Schadschneider and A.~Seyfried (2009)  {Pedestrian Behavior: Data
Collection and Applications}.\newblock In. {\em{Empirical Results
for Pedestrian Dynamics and their Implications for
  Cellular Automata Models}}.  pp. 27--43. Emerald Group Publishing
  Limited, 1st edition


\bibitem{Helbing2000}
D.~Helbing, I.~Farkas, and T.~Vicsek (2000)
\newblock {\em Nature} 407:487--490

\bibitem{Song2006}
W.~Song, X.~Xu, B.H. Wang, and S.~Ni (2006)
\newblock {\em Physica A} 363:492--500

\bibitem{Schadschneider2009a}
A.~Schadschneider, W.~Klingsch, H.~Kl\"upfel, T.~Kretz, C.~Rogsch,
and A.~Seyfried (2009) {Evacuation Dynamics: Empirical Results,
Modeling and Applications}.
\newblock In: {\em {Encyclopedia of Complexity and System Science}}, volume~5,
 (Berlin: Springer),
  pp. 3142--3176

\bibitem{Seyfried2009}
A.~Seyfried, O.~Passon, B.~Steffen, M.~Boltes, T.~Rupprecht, and
W.~Klingsch (2009)
\newblock {\em Transportation Science} 43(3):395--406

\bibitem{Tajima2002}
Y.~Tajima and T.~Nagatani (2002)
\newblock {\em Physica A} 303:239--250

\bibitem{Peng2011}
Y.C. Peng and C.I. Chou (2011)
\newblock {\em Computer Physics Communications} 182:205--208

\bibitem{Boltes2010}
M.~Boltes, A.~Seyfried, B.~Steffen, and A.~Schadschneider (2010)
\newblock {Automatic Extraction of Pedestrian Trajectories from Video
  Recordings}.
\newblock In {\em Pedestrian and Evacuation Dynamics 2008} (Berlin: Springer), pp. 43--54

\bibitem{Helbing2007}
D.~Helbing, A.~Johansson, and H.~Z. Al-Abideen (2007)
\newblock {\em Phys. Rev. E} 75:046109

\bibitem{Predtechenskii1978}
V.~M. Predtechenskii and A.~I. Milinskii (1969)
\newblock {\em {Planning for Foot Traffic Flow in Buildings}}.
\newblock Amerind Publishing, New Dehli, 1978.
\newblock Translation of: Proekttirovanie Zhdanii s Uchetom Organizatsii
  Dvizheniya Lyuddskikh Potokov, Stroiizdat Publishers, Moscow

\bibitem{Fruin1971}
J.~J. Fruin (1971)
\newblock {\em {Pedestrian Planning and Design}}.
\newblock Elevator World, New York

\bibitem{Steffen2010a}
B.~Steffen and A.~Seyfried (2010)
\newblock {\em Physica A} 389(9):1902--1910

\bibitem{Zhanga}
J.~Zhang, W.~Klingsch, A.~Schadschneider, and A.~Seyfried  (2011)
\newblock {\em J. Stat. Mech.} P06004.


\end{thebibliography}

